Adversarial Framework for Unsupervised Learning of Motion Dynamics in Videos

Human behavior understanding in videos is a complex, still unsolved problem and requires to accurately model motion at both the local (pixel-wise dense prediction) and global (aggregation of motion cues) levels. Current approaches based on supervised learning require large amounts of annotated data, whose scarce availability is one of the main limiting factors to the development of general solutions. Unsupervised learning can instead leverage the vast amount of videos available on the web and it is a promising solution for overcoming the existing limitations. In this paper, we propose an adversarial GAN-based framework that learns video representations and dynamics through a self-supervision mechanism in order to perform dense and global prediction in videos. Our approach synthesizes videos by 1) factorizing the process into the generation of static visual content and motion, 2) learning a suitable representation of a motion latent space in order to enforce spatio-temporal coherency of object trajectories, and 3) incorporating motion estimation and pixel-wise dense prediction into the training procedure. Self-supervision is enforced by using motion masks produced by the generator, as a co-product of its generation process, to supervise the discriminator network in performing dense prediction. Performance evaluation, carried out on standard benchmarks, shows that our approach is able to learn, in an unsupervised way, both local and global video dynamics. The learned representations, then, support the training of video object segmentation methods with sensibly less (about 50%) annotations, giving performance comparable to the state of the art. Furthermore, the proposed method achieves promising performance in generating realistic videos, outperforming state-of-the-art approaches especially on motion-related metrics.

==> draft.tex <==
The first part of the evaluation aimed at investigating the contribution of adversarial training for dense prediction, by assessing the quality of the foreground maps computed by our video object segmentation approach in four different training scenarios: 1) \emph{synthetic}: we extracted the segmentation subnetwork from the architecture of our discriminator and trained it from scratch, using only the fake foreground masks coming from the generator pre-trained on ``golf course''; 2) \emph{adversarial}: we trained our GAN model on the ``golf course'' dataset, then used the segmentation subnetwork from the discriminator; 3) \emph{fine-tuned synthetic}: the segmentation network trained in the \emph{synthetic} modality was then fine-tuned on ground-truth masks of the benchmark datasets' (DAVIS, SegTrack and F4K-Fish) training sets; 4) \emph{fine-tuned adversarial}: analogously, we used the segmentation model from the \emph{adversarial} training scenario fine-tuned on real segmentation masks.
